The Geometry of Adversarial Training in Binary Classification

We establish an equivalence between a family of adversarial training problems for non-parametric binary classification and a family of regularized risk minimization problems where the regularizer is a nonlocal perimeter functional. The resulting regularized risk minimization problems admit exact convex relaxations of the type $L^1+$ (nonlocal) $\operatorname{TV}$, a form frequently studied in image analysis and graph-based learning. A rich geometric structure is revealed by this reformulation which in turn allows us to establish a series of properties of optimal solutions of the original problem, including the existence of minimal and maximal solutions (interpreted in a suitable sense), and the existence of regular solutions (also interpreted in a suitable sense). In addition, we highlight how the connection between adversarial training and perimeter minimization problems provides a novel, directly interpretable, statistical motivation for a family of regularized risk minimization problems involving perimeter/total variation. The majority of our theoretical results are independent of the distance used to define adversarial attacks.

==> The Geometry of Adversarial Training/commands.tex <==
\newtheorem{theorem}{Theorem}[section]
\newtheorem*{theorem*}{Theorem}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{example}[theorem]{Example}
\theoremstyle{remark}
\newtheorem{remark}[theorem]{Remark}


\theoremstyle{definition}

\newtheorem{definition}[theorem]{Definition}
\newtheorem{assumption}{Assumption}

\numberwithin{equation}{section}

%
\newcommand{\Exp}[2]{\operatorname{\mathbb{E}}_{#1}\left[#2\right]}
\newcommand{\abs}[1]{\left|#1\right|}
\newcommand{\norm}[1]{\|#1\|}
\newcommand{\de}{\,\mathrm{d}}
\newcommand{\eps}{\varepsilon}
\newcommand{\veps}{\varepsilon}
\newcommand{\e}{\varepsilon}
\newcommand{\E}{\mathbb{E}}
\renewcommand{\rho}{\varrho}
\newcommand{\N}{\mathbb{N}}
\newcommand{\M}{\mathcal{M}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\Rd}{{\R^d}}

\newcommand{\domain}{\mathcal{X}}
\renewcommand{\P}{\mathcal{P}}

\newcommand{\B}{\mathfrak{B}}
\renewcommand{\H}{\mathcal{H}^{d-1}}
\newcommand{\st}{\,:\,}
%\DeclareMathOperator{\dist}{dist}
\newcommand{\dist}{\operatorname{\mathsf{dist}}}
\newcommand{\closure}[1]{\overline{#1}}
\newcommand{\wsto}{\rightharpoonup^\ast}
\DeclareMathOperator{\supp}{supp}
\newcommand{\loss}{\ell}

\DeclareMathOperator{\argmin}{arg\,min}


\newcommand{\metric}{\operatorname{\mathsf{d}}}

\DeclareMathOperator{\cl}{\mathsf{cl}}
\DeclareMathOperator{\op}{\mathsf{op}}
% \DeclareMathOperator{\ball}{\mathsf{B}}
\newcommand{\ball}{B}

%\newcommand{\Per}{\operatorname{Per}}
\newcommand{\PrePer}{\,\widetilde{\operatorname{Per}}}

\newcommand{\PreTV}{\,\widetilde{\operatorname{TV}}}


\newcommand{\TV}[1][]{
\ifthenelse { \equal {#1} {} }  
    {\operatorname{TV}} 
    {\operatorname{\ensuremath{#1}-TV}}
}

\newcommand{\Per}[1][]{
\ifthenelse { \equal {#1} {} }  
    {\operatorname{Per}} 
    {\operatorname{\ensuremath{#1}-Per}}
}

\newcommand{\esssup}[1][]{
\ifthenelse { \equal {#1} {} }  
    {\operatorname*{ess\,sup}} 
    {\operatorname*{\ensuremath{#1}-ess}\sup}
}
\newcommand{\essinf}[1][]{
\ifthenelse { \equal {#1} {} }  
    {\operatorname*{ess\,inf}} 
    {\operatorname*{\ensuremath{#1}-ess}\inf}
}
\newcommand{\essosc}[1][]{
\ifthenelse { \equal {#1} {} }  
    {\operatorname*{ess\,osc}} 
    {\operatorname*{\ensuremath{#1}-ess\,osc}}
}

\newcommand{\osc}{\operatorname*{osc}}

\newcommand{\restr}{\mathbin{\vrule height 1.6ex depth 0pt width
0.13ex\vrule height 0.13ex depth 0pt width 1.3ex}}

\renewcommand{\subset}{\subseteq}
\renewcommand{\supset}{\supseteq}

%colors
\newcommand{\red}{\color{red}}
\newcommand{\olive}{\color{olive}}
\newcommand{\blue}{\color{blue}}
\newcommand{\magenta}{\color{magenta}}
\newcommand{\teal}{\color{teal}}
\newcommand{\orange}{\color{orange}}
\newcommand{\nc}{\normalcolor}

%reviewers' colors
\newcommand{\first}{\blue}
\newcommand{\second}{\magenta}
\newcommand{\third}{\orange}
\renewcommand{\first}{}
\renewcommand{\second}{}
\renewcommand{\third}{}

%general edits color
\newcommand{\editscolor}{\olive}
\renewcommand{\editscolor}{}

%graphics
\graphicspath{{figures/}}

%comments
\newcommand{\off}[1]{{}}




==> The Geometry of Adversarial Training/packages.tex <==
\usepackage[T1]{fontenc}
\usepackage[utf8]{inputenc}

\usepackage{amsmath,amssymb,amsthm}
\usepackage{MnSymbol}
\usepackage{fullpage}
\setlength{\marginparwidth}{2cm}

\usepackage[
natbib,
maxcitenames=3, 
maxbibnames=10,  
sorting=ydnt,
url=false,
doi=false,
sortcites,
defernumbers,
backend=biber
]{biblatex}
\addbibresource{bibliography.bib}

\usepackage[
% colorlinks=true,
% linkcolor=blue,
% citecolor=blue
]
{hyperref}


\usepackage{tikz}

\usepackage{todonotes}

\usepackage[nameinlink, capitalise, noabbrev]{cleveref}
\usepackage[normalem]{ulem}

\usepackage{caption}
\usepackage{subcaption}


